TableLLM: Enabling Tabular Data Manipulation by LLMs in Real Office Usage Scenarios

We introduce TableLLM, a robust large language model (LLM) with 8 billion parameters, purpose-built for proficiently handling tabular data manipulation tasks, whether they are embedded within documents or spreadsheets, catering to real-world office scenarios. We propose a distant supervision method for training, which comprises a reasoning process extension strategy, aiding in training LLMs to understand reasoning patterns more effectively as well as a cross-way validation strategy, ensuring the quality of the automatically generated data. To evaluate the performance of TableLLM, we have crafted benchmarks tailored to address both document and spreadsheet formats as well as constructed a well-organized evaluation pipeline capable of handling both scenarios. Thorough evaluations underscore the advantages of TableLLM when compared to various existing general-purpose and tabular data-focused LLMs. We have publicly released the model checkpoint, source code, benchmarks, and a web application for user interaction. Our codes and data are publicly available at https://github.com/TableLLM/TableLLM.

==> latex/4.evaluation.tex <==
\begin{table}[t]
  \newcolumntype{?}{!{\vrule width 1pt}}
  \newcolumntype{C}{>{\centering\arraybackslash}p{2em}}
  \centering
  \caption{Benchmark (test set) statistics}
  \label{tb:benchmark}
  \small
  \scalebox{1.0}{
  \begin{tabular}{@{}c?c?c?c@{}}
    \toprule
    Scenario &	Name &	Description & Size \\
     \midrule
 
     \multirow{3}{*}{\tabincell{c}{Document\\-embedded}}  
     & WikiTQ  & <500 tokens \& add text & 633\\
     & FeTaQA & <500 tokens \& add text & 753\\
     & TAT-QA & <500 tokens &800\\
     & OTT-QA& <1000 tokens &1987\\

     \midrule
     \multirow{3}{*}{\tabincell{c}{Spreadsheet\\-embedded}}  
     & WikiSQL & Remove vague questions &1,000 \\
     & Spider  & Choose single table & 512  \\
     & Self-created &Query/Update/Merge/Chart &1,200 \\
    \midrule
    Both & \model-bench & - & 4,898 \\
    \bottomrule

  \end{tabular}
  }
\end{table}

We start by outlining the process of developing a benchmark for the specified problem of tabular data manipulation, followed by an introduction to the evaluation methodology.



Table~\ref{tb:benchmark} displays the benchmark statistics. The prompts used for generating questions and answers with GPT-4 are detailed in Appendix~\ref{sec:promptbenchmark}.




\subsection{Evaluation Process}
Given the diverse range of operation types in our dataset, we have adopted a categorized evaluation approach to assess the performance of models across different operations:

\begin{itemize}[leftmargin=*]
    \item \textbf{Query Operations:} For the answers obtained through code execution, we conduct an exact match comparison between the model's output and the ground truth answers to determine correctness. However, for the answers directly inferred via inner-parameters, we rely on CritiqueLLM~\cite{critiquellm} to assign a score by comparing the model's output with the ground truth answers. This is because the generated answers are often lengthy and challenging to precisely match.

    \item \textbf{Update and Merge Operations:} As these operations directly modify tables, we require the model's output to be the complete modified table. We then perform an exact match comparison between the model's output and the ground truth answers to determine correctness.
    
    \item \textbf{Chart Operations:} Assessing charting operations is challenging through direct answer comparison. Instead, we compare code output by the model with the corresponding code from the ground truth answer. Since the chart operation is exclusive to our created benchmark, the corresponding code of the ground truth answer is generated during the benchmark creation process. CritiqueLLM is once again employed to compare the model's output code with the ground truth code.
\end{itemize}

This categorized evaluation framework ensures a thorough and tailored assessment of model performance across different operation types, taking into account the complexity and unique characteristics of each task.

\begin{table}[t]
  \newcolumntype{?}{!{\vrule width 1pt}} %tapas
  \newcolumntype{C}{>{\centering\arraybackslash}p{2em}} %tapas
  \centering
  \caption{Evaluation approaches for different operations}
  \label{tb:evaluation}
  \small
  \scalebox{0.95}{
 % \begin{tabular}{@{}cccc@{}c} %tapas
  \begin{tabular}{c?c}
  \toprule
    Operations&  Approach\\
     \midrule
     Query& CritiqueLLM (compare the answers)\\
     Update& Exact match\\
 Merge&Exact match\\
     Chart& CritiqueLLM (compare the code)\\
     \bottomrule
  \end{tabular}
  }
\end{table}


